Entropic Gromov-Wasserstein between Gaussian Distributions

We study the entropic Gromov-Wasserstein and its unbalanced version between (unbalanced) Gaussian distributions with different dimensions. When the metric is the inner product, which we refer to as inner product Gromov-Wasserstein (IGW), we demonstrate that the optimal transportation plans of entropic IGW and its unbalanced variant are (unbalanced) Gaussian distributions. Via an application of von Neumann's trace inequality, we obtain closed-form expressions for the entropic IGW between these Gaussian distributions. Finally, we consider an entropic inner product Gromov-Wasserstein barycenter of multiple Gaussian distributions. We prove that the barycenter is a Gaussian distribution when the entropic regularization parameter is small. We further derive a closed-form expression for the covariance matrix of the barycenter.

==> AISTATS/macro_commands.tex <==

% Recommended, but optional, packages for figures and better typesetting:

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2018} with \usepackage[nohyperref]{icml2018} above.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath,amsfonts,bm, dsfont}
% --- For displaying two algorithms in two columns ---
%\setlength{\textwidth}{\paperwidth}
%\addtolength{\textwidth}{-6cm}
%\setlength{\textheight}{\paperheight}
%\addtolength{\textheight}{-4cm}
%\addtolength{\textheight}{-1.1\headheight}
%\addtolength{\textheight}{-\headsep}
%\addtolength{\textheight}{-\footskip}
%\setlength{\oddsidemargin}{0.5cm}
%\setlength{\evensidemargin}{0.5cm}

%\input{macro_commands.tex}
\usepackage{natbib}

%\usepackage{arxiv}

\usepackage{enumitem}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{subfigure}
\usepackage{epsf}
\usepackage{epsfig}
\usepackage{fancyhdr}
\usepackage{graphics}
\usepackage{graphicx}
% \usepackage{epstopdf}
\usepackage{psfrag}
%\usepackage{fullpage}
\usepackage{pdfpages}
%\usepackage[dvipsnames]{xcolor}

%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{url}
% for url's in bib
% for theorem hyperlink colors
%\usepackage[colorlinks,linkcolor=magenta,citecolor=blue, pagebackref=true,backref=true]{hyperref}
% \renewcommand*{\backref}[1]{\ifx#1\relax \else Page #1 \fi}
%\renewcommand*{\backrefalt}[4]{%
%    \ifcase #1 \footnotesize{(Not cited.)}%
%    \or        \footnotesize{(Cited on page~#2.)}%
%    \else      \footnotesize{(Cited on pages~#2.)}%
%    \fi}

\usepackage{url}% for url's in bib
% for theorem hyperlink colors
\usepackage[colorlinks,linkcolor=magenta,citecolor=blue, pagebackref=true,backref=true]{hyperref}
% \renewcommand*{\backref}[1]{\ifx#1\relax \else Page #1 \fi}
\renewcommand*{\backrefalt}[4]{%
    \ifcase #1 \footnotesize{(Not cited.)}%
    \or        \footnotesize{(Cited on page~#2.)}%
    \else      \footnotesize{(Cited on pages~#2.)}%
    \fi}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb,bbm}
\usepackage{caption}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{multicol}
\usepackage{caption}
%\captionsetup[algorithm]{singlelinecheck=off}
\usepackage{color}
%\usepackage{biblatex}
%\addbibresource{refs.bib}
%\bibliographystyle{abbrv}

\usepackage{changes}
\definechangesauthor[name=Huy Nguyen, color=purple]{HN}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\id}{Id}
\DeclareMathOperator{\cov}{Cov}

% \newtheorem{assumption}{Assumption}
% \newtheorem{remark}{Remark}
% \newtheorem{observation}{Observation}
% \newtheorem{lemma}{Lemma}
% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{definition}{Definition}
% \newtheorem{corollary}{Corollary}



%\newcommand{\dim}{\textnormal{dim}}

\newenvironment{assumptionprime}[1]
  {\renewcommand{\theassumption}{\ref{#1}$'$}%
   \addtocounter{assumption}{-1}%
   \begin{assumption}}
  {\end{assumption}}

\newcommand{\genecomment}[1]{{\bf{{\blue{{TEAM --- #1}}}}}}
% --- For coloring ---
\usepackage{changes}



\renewcommand\arraystretch{1.5}




\def\st{\textnormal{s.t.}}
\def\sgn{\texttt{sign}}

\def\GW{{\mathds{GW}}}
\def\GGW{{\mathds{GGW}}}
\def\UGW{{\mathcal{UGW}}}
\def\GTW{{\mathcal{GW}_{T}}}
\def\TGW{{\mathcal{GW}_{T}}}


\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\CC{\mathbf{C}}
\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
%\def\FF{\mathbb{F}}


\def\Xx{\mathcal{X}}
\def\Yy{\mathcal{Y}}
\def\Tt{\mathcal{T}}
\def\Nn{\mathcal{N}}
\def\Ff{\mathcal{F}}
\def\Bb{\mathcal{B}}
\def\Gg{\mathcal{G}}
\def\Dd{\mathcal{D}}

\def\E{\mathbb{E}}

\def\EE{\mathbb{E}}
\def\RR{\mathbb{R}}
\def\dd{\mathrm{d}}

\def\KLO{\mathcal{O}_{\mathrm{KL}}}
\def\GWO{\mathcal{O}_{\mathrm{GW}}}
\def\WO{\mathcal{O}_{\mathrm{W}}}

\def\Sigmax{\Sigma_{x}}
\def\Sigmay{\Sigma_{y}}
% \def\Sigmaxy{\Sigma_{xy}}
\def\Sigmaxy{K}
\def\diag{\mathrm{diag}}
\def\Diag{\mathrm{Diag}}

\def\aA{\mathbf{a}}
\def\bB{\mathbf{b}}
\def\pP{\mathbf{p}}
\def\qQ{\mathbf{q}}
\def\rR{\mathbf{r}}
\def\uU{\mathbf{u}}
\def\vV{\mathbf{v}}
\def\sS{\mathbf{s}}

\def\trace{\mathrm{trace}} %trace of  matrix
\def\det{\mathrm{det}} % determinant of a matrix




==> macro_commands.tex <==

% Recommended, but optional, packages for figures and better typesetting:

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2018} with \usepackage[nohyperref]{icml2018} above.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath,amsfonts,bm, dsfont}
% --- For displaying two algorithms in two columns ---
%\setlength{\textwidth}{\paperwidth}
%\addtolength{\textwidth}{-6cm}
%\setlength{\textheight}{\paperheight}
%\addtolength{\textheight}{-4cm}
%\addtolength{\textheight}{-1.1\headheight}
%\addtolength{\textheight}{-\headsep}
%\addtolength{\textheight}{-\footskip}
%\setlength{\oddsidemargin}{0.5cm}
%\setlength{\evensidemargin}{0.5cm}

\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-6cm}
\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-4cm}
\addtolength{\textheight}{-1.1\headheight}
\addtolength{\textheight}{-\headsep}
\addtolength{\textheight}{-\footskip}
\setlength{\oddsidemargin}{0.5cm}
\setlength{\evensidemargin}{0.5cm}

%\input{macro_commands.tex}
\usepackage{natbib}

%\usepackage{arxiv}

\usepackage{enumitem}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{subfigure}
\usepackage{epsf}
\usepackage{epsfig}
\usepackage{fancyhdr}
\usepackage{graphics}
\usepackage{graphicx}
% \usepackage{epstopdf}
\usepackage{psfrag}
%\usepackage{fullpage}
\usepackage{pdfpages}
%\usepackage[dvipsnames]{xcolor}

%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{url}
% for url's in bib
% for theorem hyperlink colors
%\usepackage[colorlinks,linkcolor=magenta,citecolor=blue, pagebackref=true,backref=true]{hyperref}
% \renewcommand*{\backref}[1]{\ifx#1\relax \else Page #1 \fi}
%\renewcommand*{\backrefalt}[4]{%
%    \ifcase #1 \footnotesize{(Not cited.)}%
%    \or        \footnotesize{(Cited on page~#2.)}%
%    \else      \footnotesize{(Cited on pages~#2.)}%
%    \fi}

\usepackage{url}% for url's in bib
% for theorem hyperlink colors
\usepackage[colorlinks,linkcolor=magenta,citecolor=blue, pagebackref=true,backref=true]{hyperref}
% \renewcommand*{\backref}[1]{\ifx#1\relax \else Page #1 \fi}
\renewcommand*{\backrefalt}[4]{%
    \ifcase #1 \footnotesize{(Not cited.)}%
    \or        \footnotesize{(Cited on page~#2.)}%
    \else      \footnotesize{(Cited on pages~#2.)}%
    \fi}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb,bbm}
\usepackage{caption}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{multicol}
\usepackage{caption}
%\captionsetup[algorithm]{singlelinecheck=off}
\usepackage{color}
%\usepackage{biblatex}
%\addbibresource{refs.bib}
%\bibliographystyle{abbrv}

\usepackage{changes}
\definechangesauthor[name=Huy Nguyen, color=purple]{HN}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\id}{Id}
\DeclareMathOperator{\cov}{Cov}

\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{observation}{Observation}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}



%\newcommand{\dim}{\textnormal{dim}}

\newenvironment{assumptionprime}[1]
  {\renewcommand{\theassumption}{\ref{#1}$'$}%
   \addtocounter{assumption}{-1}%
   \begin{assumption}}
  {\end{assumption}}

\newcommand{\genecomment}[1]{{\bf{{\blue{{TEAM --- #1}}}}}}
% --- For coloring ---
\usepackage{changes}



\renewcommand\arraystretch{1.5}




\def\st{\textnormal{s.t.}}
\def\sgn{\texttt{sign}}

\def\GW{{\mathds{GW}}}
\def\GGW{{\mathds{GGW}}}
\def\UGW{{\mathcal{UGW}}}
\def\GTW{{\mathcal{GW}_{T}}}
\def\TGW{{\mathcal{GW}_{T}}}


\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\CC{\mathbf{C}}
\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
%\def\FF{\mathbb{F}}


\def\Xx{\mathcal{X}}
\def\Yy{\mathcal{Y}}
\def\Tt{\mathcal{T}}
\def\Nn{\mathcal{N}}
\def\Ff{\mathcal{F}}
\def\Bb{\mathcal{B}}
\def\Gg{\mathcal{G}}
\def\Dd{\mathcal{D}}

\def\E{\mathbb{E}}

\def\EE{\mathbb{E}}
\def\RR{\mathbb{R}}
\def\dd{\mathrm{d}}

\def\KLO{\mathcal{O}_{\mathrm{KL}}}
\def\GWO{\mathcal{O}_{\mathrm{GW}}}
\def\WO{\mathcal{O}_{\mathrm{W}}}

\def\Sigmax{\Sigma_{x}}
\def\Sigmay{\Sigma_{y}}
% \def\Sigmaxy{\Sigma_{xy}}
\def\Sigmaxy{K}
\def\diag{\mathrm{diag}}
\def\Diag{\mathrm{Diag}}

\def\aA{\mathbf{a}}
\def\bB{\mathbf{b}}
\def\pP{\mathbf{p}}
\def\qQ{\mathbf{q}}
\def\rR{\mathbf{r}}
\def\uU{\mathbf{u}}
\def\vV{\mathbf{v}}
\def\sS{\mathbf{s}}

\def\trace{\mathrm{trace}} %trace of  matrix
\def\det{\mathrm{det}} % determinant of a matrix



